Multiple backscattering in trivial and non-trivial topological photonic crystal edge states with controlled disorder

We present an experimental investigation of multiple scattering in photonic-crystal-based topological edge states with and without engineered random disorder. We map the spatial distribution of light as it propagates along a so-called bearded interface between two valley photonic crystals which supports both trivial and non-trivial edge states. As the light slows down and/or the disorder increases, we observe the photonic manifestation of Anderson localization, illustrated by the appearance of localized high-intensity field distributions. We extract the backscattering mean free path (BMFP) as a function of frequency, and thereby group velocity, for a range of geometrically engineered random disorders of different types. For relatively high group velocities (with $n_g < 15$), we observe that the BMFP is an order of magnitude higher for the non-trivial edge state than for the trivial. However, the BMFP for the non-trivial mode decreases rapidly with increasing disorder. As the light slows down the BMFP for the trivial state decreases as expected, but the BMFP for the topological state exhibits a non-conventional dependence on the group velocity. Due to the particular dispersion of the topologically non-trivial mode, a range of frequencies exist where two distinct states can have the same group index but exhibit a different BMFP. While the topological mode is not immune to backscattering at disorder that breaks the protecting crystalline symmetry, it displays a larger robustness than the trivial mode for a specific range of parameters in the same structure. Intriguingly, the topologically non-trivial edge state appears to break the conventional relationship between slowdown and the amount of backscattering.

==> Summary.tex <==
%Popular Summary
% 250 words in length


Topological photonic crystals hold immense promise for revolutionizing on-chip photonic devices by creating one-way pathways for light, offering precise control over light-matter interactions. This research addresses a crucial question: How robust are these unidirectional pathways when confronted with unexpected disorders and how can we harness the power of these unidirectional pathways to enhance our technology? 

The scientists started by intentionally adding randomness by perturbing the positions and sizes of the crystal's "holes," akin to navigating a pathway strewn with obstacles. Disorder,  as expected, impacts the road's ability to facilitate light flow, presenting two scenarios: an ideal, smooth, and clear road versus a bumpy, winding one.

Within these pathways, two types of light carriers emerge: one seemingly resilient and another more susceptible to disruption. Initially, the resilient carrier stands strong against the chaos, while the traditionally weaker one starts showing signs faltering. However, as the disorder intensities, both carriers begin to falter, eventually succumbing to a complete stop known as Anderson localization. 

What this mean for the future of photonics is that even the best navigation system has limits. This research reminds us that while topological protection is impressive, it's not a magic bullet. We need to consider disorder and other unforeseen factors when designing photonic devices. This research underscores a crucial insight for the future of photonics: even the most sophisticated navigation system has limitations. While topological protection is impressive, when designing photonic devices, we must account for unforeseen factors such as ubiquitous disorders. 




